Benchmarking near-term quantum devices with the Variational Quantum Eigensolver and the Lipkin-Meshkov-Glick model

The Variational Quantum Eigensolver (VQE) is a promising algorithm for Noisy Intermediate Scale Quantum (NISQ) computation. Verification and validation of NISQ algorithms' performance on NISQ devices is an important task. We consider the exactly-diagonalizable Lipkin-Meshkov-Glick (LMG) model as a candidate for benchmarking NISQ computers. We use the Bethe ansatz to construct eigenstates of the trigonometric LMG model using quantum circuits inspired by the LMG's underlying algebraic structure. We construct circuits with depth $\mathcal{O}(N)$ and $\mathcal{O}(\log_2N)$ that can prepare any trigonometric LMG eigenstate of $N$ particles. The number of gates required for both circuits is $\mathcal{O}(N)$. The energies of the eigenstates can then be measured and compared to the exactly-known answers.

==> macros.tex <==
\newcommand{\twopartdef}[3]
{
	\left\{
		\begin{array}{lll}
			#1 & \mbox{if } #2 \\
			#3 & \mbox{otherwise } 
		\end{array}
	\right.
}
\newcommand{\Soln}{\noindent{\bf Solution}}
\newcommand{\csch}{{\rm csch}}
\newcommand{\sech}{{\rm sech}}
\newcommand{\T}{(Townsend)~}
\newcommand{\In}{Individual:~}
\newcommand{\G}{Group:~}
\newcommand{\NC}{{\bf Extra information not required for credit:}~}
\newcommand{\TP}{{\bf Total:}~}
\newcommand{\PO}{{\bf (1 Point)}~}
\newcommand{\PT}{{\bf (2 Points)}~}
\newcommand{\PTh}{{\bf (3 Points)}~}
\newcommand{\PF}{{\bf (4 Points)}~}
\newcommand{\PFi}{{\bf (5 Points)}~}
\newcommand{\PS}{{\bf (6 Points)}~}
\newcommand{\PSe}{{\bf (7 Points)}~}
\newcommand{\PE}{{\bf (8 Points)}~}
\newcommand{\PN}{{\bf (9 Points)}~}
\newcommand{\PTe}{{\bf (10 Points)}~}
\newcommand{\PEl}{{\bf (11 Points)}~}
\newcommand{\PTwe}{{\bf (12 Points)}~}
\newcommand{\PThi}{{\bf (13 Points)}~}
\newcommand{\PFo}{{\bf (14 Points)}~}
\newcommand{\PFif}{{\bf (15 Points)}~}
\newcommand{\PSi}{{\bf (16 Points)}~}
\newcommand{\RP}{{\bf Relevant problems:}~}
\newcommand{\AP}{{\bf Assigned problems:}~}
\def\ket#1{\left\vert #1 \right\rangle}
\def\bra#1{\left\langle #1 \right\vert}
\def\braket#1#2{\left\langle #1 \vert #2\right\rangle}
\newcommand{\kpz}{\ket{+{\bfz}}}
\newcommand{\kmz}{\ket{-{\bfz}}}
\newcommand{\bpz}{\bra{+{\bfz}}}
\newcommand{\bmz}{\bra{-{\bfz}}}
\newcommand{\kpx}{\ket{+{\bfx}}}
\newcommand{\kmx}{\ket{-{\bfx}}}
\newcommand{\bpx}{\bra{+{\bfx}}}
\newcommand{\bmx}{\bra{-{\bfx}}}
\newcommand{\kpy}{\ket{+{\bfy}}}
\newcommand{\kmy}{\ket{-{\bfy}}}
\newcommand{\bpy}{\bra{+{\bfy}}}
\newcommand{\bmy}{\bra{-{\bfy}}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bp}{\begin{pmatrix}}
\newcommand{\ep}{\end{pmatrix}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\px}{\bp0&1\\1&0\ep}
\newcommand{\py}{\bp0&-i\\i&0\ep}
\newcommand{\pz}{\bp1&0\\0&-1\ep}
\newcommand{\id}{\bp1&0\\0&1\ep}
\newcommand{\pxpx}{\bp0&0&0&1\\0&0&1&0\\0&1&0&0\\1&0&0&0\ep}
\newcommand{\pypy}{\bp0&0&0&-1\\0&0&1&0\\0&1&0&0\\ -1&0&0&0\ep}
\newcommand{\pzpz}{\bp1&0&0&0\\0&-1&0&0\\0&0&-1&0\\0&0&0&1\ep}
\newcommand{\emf}{{\cal E}}
\newcommand{\bfE}{{\bf E}}
\newcommand{\bfB}{{\bf B}}
\newcommand{\bfn}{{\bf n}}
\newcommand{\bfdl}{{\bf dl}}
\newcommand{\bfdA}{{\bf dA}}
\newcommand{\bfp}{{\bf p}}
\newcommand{\bfr}{{\bf r}}
\newcommand{\bfi}{{\bf i}}
\newcommand{\bfj}{{\bf j}}
\newcommand{\bfk}{{\bf k}}
\newcommand{\iot}{i\omega t}
\newcommand{\eiot}{e^{i\omega t}}
\newcommand{\bfe}{{\bf e}}
\newcommand{\bfc}{{\bf c}}
\newcommand{\bfcj}{\bfc_j}
\newcommand{\cja}{c_{j\alpha}}
\newcommand{\cjb}{c_{j\beta}}
\newcommand{\cjc}{c_{jP}}
\newcommand{\cjd}{c_{j\delta}}
\newcommand{\bfu}{{\bf u}}
\newcommand{\bfv}{{\bf v}}
\newcommand{\bfN}{{\bf N}}
\newcommand{\bfx}{{\bf x}}
\newcommand{\bfy}{{\bf y}}
\newcommand{\bfz}{{\bf z}}
\newcommand{\bfZ}{{\bf Z}}
\newcommand{\Neq}{{N^{\mbox{\scriptsize eq}}}}
\newcommand{\dt}{{\Delta t}}
\newcommand{\bfbeta}{{\mbox{\boldmath $\beta$}}}
\newcommand{\bfzero}{{\mbox{\boldmath $0$}}}
\newcommand{\bfone}{{\mbox{\boldmath $1$}}}
\newcommand{\bfnabla}{{\mbox{\boldmath $\nabla$}}}
\newcommand{\LamInv}{{\mbox{$\Lambda^{-1}$}}}
\newcommand{\LamInvT}{{\mbox{$\Lambda^{-1}$}^T}}
\newcommand{\taumin}{{\tau_{\mbox{\tiny $\min$}}}}
\newcommand{\rhoomb}{{\frac{\rho}{mb}}}
\newcommand{\phip}{{\phi'\left(\rhoomb\right)}}
\newcommand{\phipp}{{\phi''\left(\rhoomb\right)}}
\newcommand{\phipx}{{\phi'\left(x\right)}}
\newcommand{\phippx}{{\phi''\left(x\right)}}

